Error-detected state transfer and entanglement in a superconducting quantum network

Modular networks are a promising paradigm for increasingly complex quantum devices based on the ability to transfer qubits and generate entanglement between modules. These tasks require a low-loss, high-speed intermodule link that enables extensible network connectivity. Satisfying these demands simultaneously remains an outstanding goal for long-range optical quantum networks as well as modular superconducting processors within a single cryostat. We demonstrate communication and entanglement in a superconducting network with a microwave-actuated beamsplitter transformation between two bosonic qubits, which are housed in separate modules and joined by a demountable coaxial bus resonator. We transfer a qubit in a multi-photon encoding and track photon loss events to improve the fidelity, making it as high as in a single-photon encoding. Furthermore, generating entanglement with two-photon interference and postselection against loss errors produces a Bell state with success probability 79% and fidelity 0.94, halving the error obtained with a single photon. These capabilities demonstrate several promising methods for faithful operations between modules, including novel possibilities for resource-efficient direct gates.

==> author_contribs.tex <==

\section*{Author Contributions}
L.D.B. and J.T. designed the experiment with input from Y.Z., C.J.A., and R.J.S.
L.D.B. and J.T. performed the experiment and analyzed the data under the supervision of R.J.S.
L.D.B. and L.F. fabricated the transmon qubits.
L.J., M.D., and S.M.G. provided theoretical support.
L.D.B., J.T., and R.J.S. wrote the manuscript with input from all authors.
